Online Generation of Proofs Without Words

Understanding geometric relationships with little mathematical knowledge can be challenging for today's students and teachers. A new toolset is introduced that is able to create a proof without words by combining the benefits of the Geometric Deduction Database method (to obtain a readable proof of a geometric statement) and the GeoGebra framework (that makes it possible to export these data as an online applet in a simple way).

==> eptcsdata.tex <==
\providecommand{\firstpage}{103}
\providecommand{\publicationstatus}{Jani\v{c}i\'c, Kov\'acs (Eds.): Automated Deduction in Geometry (ADG 2021)\\
EPTCS 352, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.352.10}{10.4204/EPTCS.352.10}}
\pdfoutput=1

